Understanding the Role of the Projector in Knowledge Distillation

In this paper we revisit the efficacy of knowledge distillation as a function matching and metric learning problem. In doing so we verify three important design decisions, namely the normalisation, soft maximum function, and projection layers as key ingredients. We theoretically show that the projector implicitly encodes information on past examples, enabling relational gradients for the student. We then show that the normalisation of representations is tightly coupled with the training dynamics of this projector, which can have a large impact on the students performance. Finally, we show that a simple soft maximum function can be used to address any significant capacity gap problems. Experimental results on various benchmark datasets demonstrate that using these insights can lead to superior or comparable performance to state-of-the-art knowledge distillation techniques, despite being much more computationally efficient. In particular, we obtain these results across image classification (CIFAR100 and ImageNet), object detection (COCO2017), and on more difficult distillation objectives, such as training data efficient transformers, whereby we attain a 77.2% top-1 accuracy with DeiT-Ti on ImageNet. Code and models are publicly available.

==> tables/augmentation.tex <==
\resizebox{1.\linewidth}{!}{
\begin{tabular}{llcc}
    \toprule
    Description & Loss paths & acc@1 & acc@5 \\
    \midrule
    KD & \multicolumn{1}{m{3.1cm}}{\includegraphics[scale=0.5]{papers/rethinking_distillation/figures/zs_zt.pdf}} & - & - \\
    % \midrule
    KD + SS & \multicolumn{1}{m{3.1cm}}{\includegraphics[scale=0.5]{papers/rethinking_distillation/figures/zs_zt_zs_zsd.pdf}} & - & - \\
    \midrule
\end{tabular}
\quad
\begin{tabular}{llcc}
    \toprule
    Description & Loss paths & acc@1 & acc@5 \\
    \midrule
    Augment & \multicolumn{1}{m{3.1cm}}{\includegraphics[scale=0.5]{papers/rethinking_distillation/figures/zs_zt_zs_ztd.pdf}} & - & - \\
    % \midrule
    Cross-augment & \multicolumn{1}{m{3.1cm}}{\includegraphics[scale=0.5]{papers/rethinking_distillation/figures/zs_zt_cross.pdf}} & - & - \\
    \midrule
\end{tabular}
}

==> tables/capacity_gap.tex <==
\begin{tabular}{lccc}
    \toprule
    Loss & acc@1 \\
    \midrule
    MSE & 70.03 \\
    \myalign{l}{\;\;\;\footnotesize $\rotatebox[origin=c]{180}{$\Lsh$}$ w/ BN + LogSum} & 71.29 \\
    \midrule
\end{tabular}

==> tables/cifar100_no_aug.tex <==
\setlength\tabcolsep{5pt}
\resizebox{1.0\textwidth}{!}{\begin{tabular}{c|ccccccc|cccccc}
    \toprule
    \textbf{Teacher} & \cellcolor{sarch}\textbf{W40-2} &  \cellcolor{sarch} \cellcolor{sarch}\textbf{W40-2} &  \cellcolor{sarch}\textbf{R56} &  \cellcolor{sarch}\textbf{R110} &  \cellcolor{sarch}\textbf{R110} &  \cellcolor{sarch}\textbf{R32x4} &  \cellcolor{sarch}\textbf{V13} & \cellcolor{xarch}\textbf{V13} & \cellcolor{xarch}\textbf{R50} & \cellcolor{xarch}\textbf{R50} & \cellcolor{xarch}\textbf{R32x4} & \cellcolor{xarch}\textbf{R32x4} & \cellcolor{xarch}\textbf{W40-2} \\
    \textbf{Student} &  \cellcolor{sarch}\textbf{W16-2} &  \cellcolor{sarch}\textbf{W40-1} &  \cellcolor{sarch}\textbf{R20} &  \cellcolor{sarch}\textbf{R20} &  \cellcolor{sarch}\textbf{R32} &  \cellcolor{sarch}\textbf{R8x4} &  \cellcolor{sarch}\textbf{V8} &  \cellcolor{xarch}\textbf{MN2} & \cellcolor{xarch}\textbf{MN2} & \cellcolor{xarch}\textbf{V8} & \cellcolor{xarch}\textbf{SN1} & \cellcolor{xarch}\textbf{SN2} & \cellcolor{xarch}\textbf{SN1}\\
    \midrule
    Teacher & 75.61 & 75.61 & 72.32 & 74.31 & 74.31 & 79.42 & 74.64 & 74.64 & 79.34 & 79.34 & 79.42 & 79.42 & 75.61 \\ 
    Student & 73.26 & 71.98 & 69.06 & 69.06 & 71.14 & 72.50 & 70.36 & 64.60 & 64.60 & 70.36 & 70.50 & 71.82 & 70.50 \\ 
    \midrule
    KD~\cite{Hinton2015DistillingNetwork} & 74.92 & 73.54 & 70.66 & 70.67 & 73.08 & 73.33 & 72.98 & 67.37 & 67.35 & 73.81 & 74.07 & 74.45 & 74.83\\
    FitNet~\cite{Romero2015FitNets:Nets} & 73.58  & 72.24  & 69.21  & 68.99  & 71.06  & 73.50  & 71.02 & 64.14  & 63.16  & 70.69  & 73.59  & 73.54  & 73.73  \\
    AT~\cite{Zagoruyko2019PayingTransfer} & 74.08  & 72.77  & 70.55  & 70.22  & 72.31  & 73.44  & 71.43 & 59.40  & 58.58  & 71.84  & 71.73  & 72.73  & 73.32  \\
    SP~\cite{Tung2019Similarity-preservingDistillation} & 73.83  & 72.43  & 69.67  & 70.04  & 72.69  & 72.94  & 72.68 & 66.30  & 68.08  & 73.34  & 73.48  & 74.56  & 74.52 \\
    CC~\cite{Peng2019CorrelationDistillation} & 73.56  & 72.21  & 69.63  & 69.48  & 71.48  & 72.97  & 70.71 & 64.86  & 65.43  & 70.25  & 71.14  & 71.29  & 71.38 \\
    %VID~\cite{Ahn2019VariationalTransfer} & 74.11  & 73.30  & 70.38  & 70.16  & 72.61  & 73.09  & 71.23 & 65.56  & 67.57  & 70.30  & 73.38  & 73.40  & 73.61  \\
    RKD~\cite{Park2019RelationalDistillation} & 73.35  & 72.22  & 69.61  & 69.25  & 71.82  & 71.90  & 71.48 & 64.52  & 64.43  & 71.50  & 72.28  & 73.21  & 72.21 \\
    PKT~\cite{Passalis2018LearningTransfer} & 74.54  & 73.45  & 70.34  & 70.25  & 72.61  & 73.64  & 72.88 & 67.13  & 66.52  & 73.01  & 74.10  & 74.69  & 73.89  \\
    %AB~\cite{Heo2019KnowledgeNeurons} & 72.50  & 72.38  & 69.47  & 69.53  & 70.98  & 73.17  & 70.94 & 66.06  & 67.20  & 70.65  & 73.55  & 74.31  & 73.34  \\
    FT~\cite{Kim2018ParaphrasingTransfer} & 73.25  & 71.59  & 69.84  & 70.22  & 72.37  & 72.86  & 70.58 & 61.78  & 60.99  & 70.29  & 71.75  & 72.50  & 72.03 \\
    % FSP~\cite{Yim2017ALearning} & 72.91  & n/a & 69.95  & 70.11  & 71.89  & 72.62  & 70.23  \\
    NST~\cite{Huang2017LikeTransfer} & 73.68  & 72.24  & 69.60  & 69.53  & 71.96  & 73.30  & 71.53 & 58.16  & 64.96  & 71.28  & 74.12  & 74.68  & 74.89 \\
    
    % CRD~\cite{Tian2019ContrastiveDistillation} & 75.48  & 74.14  & 71.16  & 71.46  & 73.48  & 75.51  & 73.94 & 69.73  & 69.11  & 74.30  & 75.11  & 75.65  & 76.05 \\
    % CRD+KD~\cite{Tian2019ContrastiveDistillation} & 75.64  & 74.38  & 71.63  & 71.56  & 73.75  & 75.46  & 74.29 & 69.94  & 69.54  & 74.58  & 75.12  & 76.05  & 76.27  \\
    % Just reporting their +KD
    CRD~\cite{Tian2019ContrastiveDistillation} & 75.64  & 74.38  & 71.63  & 71.56  & 73.75  & 75.46  & 74.29 & 69.94  & 69.54  & 74.58  & 75.12  & 76.05  & 76.27  \\
    
    % WCoRD~\cite{Chen2020WassersteinDistillation} & 75.88  & 74.73  & 71.56  & 71.57  & 73.81  & 75.95  & 74.55 & 69.47  & 70.45  & 74.86  & 75.40  & 75.96  & 76.32 \\
    % WCoRD+KD~\cite{Chen2020WassersteinDistillation} & 76.11  & 74.72  & \textbf{71.92}  & \underline{71.88}  & \underline{74.20}  & \underline{76.15}  & 74.72 & 70.02  & 70.12  & 74.68  & 75.77  & 76.48  & 76.68   \\
    
    % Just reporting their +KD
    WCoRD~\cite{Chen2020WassersteinDistillation} & \underline{76.11}  & 74.72  & \textbf{71.92}  & \underline{71.88}  & \underline{74.20}  & \underline{76.15}  & 74.72 & 70.02  & 70.12  & 74.68  & 75.77  & 76.48  & 76.68   \\
    
    ReviewKD~\cite{Chen2021DistillingReview} & \textbf{76.12}  & \underline{75.09}  & \underline{71.89}  & -  & 73.89  & 75.63  & \underline{74.84} & \underline{70.37}  & 69.89  & - & \textbf{77.45}  & \textbf{77.78}  & \underline{77.14} \\
    
    \midrule
    $\mathcal{L}_{corr}$ & 
    \stackengine{2pt}{75.85}{$_{\pm 0.12}$}{U}{c}{F}{T}{S} & 
    \stackengine{2pt}{74.90}{$_{\pm 0.29}$}{U}{c}{F}{T}{S} & 
    \stackengine{2pt}{71.45}{$_{\pm 0.21}$}{U}{c}{F}{T}{S} & 
    \stackengine{2pt}{71.77}{$_{\pm 0.34}$}{U}{c}{F}{T}{S} & 
    \stackengine{2pt}{74.02}{$_{\pm 0.27}$}{U}{c}{F}{T}{S} &
    \stackengine{2pt}{75.63}{$_{\pm 0.09}$}{U}{c}{F}{T}{S} & 
    \stackengine{2pt}{74.70}{$_{\pm 0.27}$}{U}{c}{F}{T}{S} &  
    \stackengine{2pt}{69.97}{$_{\pm 0.33}$}{U}{c}{F}{T}{S}  & 
    \stackengine{2pt}{\textbf{71.41}}{$_{\pm 0.41}$}{U}{c}{F}{T}{S}  & 
    \stackengine{2pt}{\textbf{75.71}}{$_{\pm 0.02}$}{U}{c}{F}{T}{S} & 
    \stackengine{2pt}{76.80}{$_{\pm 0.28}$}{U}{c}{F}{T}{S} &
    \stackengine{2pt}{77.27}{$_{\pm 0.25}$}{U}{c}{F}{T}{S} &
    \stackengine{2pt}{\textbf{77.35}}{$_{\pm 0.25}$}{U}{c}{F}{T}{S} \\  

    $\mathcal{L}_{corr}+\mathcal{L}_{mi}$ & 
    \stackengine{2pt}{\textbf{76.12}}{$_{\pm 0.04}$}{U}{c}{F}{T}{S} & 
    \stackengine{2pt}{\textbf{75.18}}{$_{\pm 0.22}$}{U}{c}{F}{T}{S} & 
    \stackengine{2pt}{{71.47}}{$_{\pm 0.07}$}{U}{c}{F}{T}{S} & 
    \stackengine{2pt}{\textbf{71.99}}{$_{\pm 0.46}$}{U}{c}{F}{T}{S} & 
    \stackengine{2pt}{\textbf{74.26}}{$_{\pm 0.05}$}{U}{c}{F}{T}{S} &
    \stackengine{2pt}{\textbf{76.19}}{$_{\pm 0.22}$}{U}{c}{F}{T}{S} & 
    \stackengine{2pt}{\textbf{74.93}}{$_{\pm 0.12}$}{U}{c}{F}{T}{S} & 
    \stackengine{2pt}{\textbf{70.39}}{$_{\pm 0.39}$}{U}{c}{F}{T}{S} & 
    \stackengine{2pt}{\underline{71.34}}{$_{\pm 0.33}$}{U}{c}{F}{T}{S}  & \stackengine{2pt}{\underline{75.49}}{$_{\pm 0.32}$}{U}{c}{F}{T}{S}  & 
    \stackengine{2pt}{\underline{76.91}}{$_{\pm 0.19}$}{U}{c}{F}{T}{S} & 
    \stackengine{2pt}{\underline{77.40}}{$_{\pm 0.06}$}{U}{c}{F}{T}{S} &
    \stackengine{2pt}{77.09}{$_{\pm 0.08}$}{U}{c}{F}{T}{S} \\    

    \midrule

    Ours & - & - & - & - & - & - & - & 71.00 & 71.30 & 75.51 & 76.73 & 77.83 & 77.14 \\

    Ours & - & - & - & - & - & - & - & 69.52 & 70.04 & 74.94 & 76.04 & 77.17 & 76.40 \\

    % Linear + KL [T=4]
    Ours & - & - & - & - & - & - & - & 69.52 & 70.25 & 74.48 & 77.15 & 76.94 & 76.64 \\

    % Linear + new KL [T=4]
    Ours & - & - & - & - & - & - & - & - & - & - & 76.55 & - & - \\

    % MLP + new KL [T=4]
    Ours & - & - & - & - & - & - & - & - & - & - & - & - & - \\
    
    \bottomrule
    \end{tabular}}

==> tables/deit.tex <==
\begin{tabular}{lccc}
    \toprule
    Network & acc@1	& acc@5	& \#params \\
    \midrule
    RegNety 160~\cite{Radosavovic2020DesigningSpaces} & 82.6 & 96.4 & 84M \\

    \midrule
    DeiT-Ti~\cite{Touvron2021TrainingAttention} & 72.2 & 91.1 & 5M\\
    DeiT-Ti\alambic\xspace ~\cite{Touvron2021TrainingAttention} & 74.5 & 91.9 & 6M \\
    DeiT-Ti\alambic\xspace 1000 epochs & 76.6 & - & 6M \\
    $\rotatebox[origin=c]{180}{$\Lsh$}$ Co-advise~\cite{Ren2022Co-advise:Distillation} & 74.9 & - & 6M \\
    $\rotatebox[origin=c]{180}{$\Lsh$}$ DearKD~\cite{chen2022dearkd} & 74.8 & - & 6M \\
    $\rotatebox[origin=c]{180}{$\Lsh$}$ DearKD - 1000 epochs & 77.0 & - & 6M \\
    $\rotatebox[origin=c]{180}{$\Lsh$}$ USKD~\cite{yang2023knowledge} & 75.0 & - & 6M \\
    % best checkpoint is 77.2
    $\rotatebox[origin=c]{180}{$\Lsh$}$ Our Method & \textbf{77.2} & \textbf{93.7} & 6M \\
    \midrule

    ResNet-50 & 76.5 & - & 25M \\
    $\rotatebox[origin=c]{180}{$\Lsh$}$ FunMatch~\cite{Beyer2022KnowledgeConsistent} & 80.3 & - & 25M \\
    $\rotatebox[origin=c]{180}{$\Lsh$}$ FunMatch - 9600 epochs & 82.3 & - & 25M \\
    Swin-Ti & 81.3 & - & 29M \\ \vspace{0.3em}
    $\rotatebox[origin=c]{180}{$\Lsh$}$ DIST$^\dagger$~\cite{huang2022knowledge} & 82.3 & - & 29M \\
    \midrule
    
    DeiT-S~\cite{Touvron2021TrainingAttention} & 79.8 & 95.0 & 22M \\
    DeiT-S\alambic\xspace ~\cite{Touvron2021TrainingAttention} & 81.2 & 95.4 & 22M \\
    $\rotatebox[origin=c]{180}{$\Lsh$}$ Co-advise~\cite{Ren2022Co-advise:Distillation} & 82.0 & - & 22M \\
    $\rotatebox[origin=c]{180}{$\Lsh$}$ DearKD~\cite{chen2022dearkd} & 81.5 & - & 22M \\
    $\rotatebox[origin=c]{180}{$\Lsh$}$ USKD~\cite{yang2023knowledge} & 80.8 & - & 22M \\
    % one ckpt is 82.1
    $\rotatebox[origin=c]{180}{$\Lsh$}$ Our Method & \textbf{82.1} & \textbf{96.0} & 22M \\
    % DeiT-S-ITRD++ & - & - & 22M \\
    \midrule
\end{tabular}

==> tables/deit_new.tex <==
\begin{tabular}{lccc}
    
    \toprule
    \belowrulesepcolor{mygrey} 
    \rowcolor{mygrey} Network & acc@1 & Teacher & \#params \\
    \aboverulesepcolor{mygrey}
    \midrule
    RegNetY-160 & 82.6 & none & 84M \\
    % 236,335,208
    BiT-M R152x2 & 84.5 & none & 236M \\
    % ~\cite{Radosavovic2020DesigningSpaces}
    % CaiT-S24~\cite{touvron2021going} & 83.4 & none & 47M \\
    % DeiT3-B~\cite{touvron2022deit} & \textbf{83.8} & none & 87M \\
    % CeiT-S~\cite{yuan2021incorporating} \textit{\footnotesize ICCV21} & 83.3 & none & 24M \\
    % ResNet101 & - & none & -M \\
    % \midrule
    % ViT-B~\cite{dosovitskiy2021an} \textit{\footnotesize ICLR21} & 77.9 & none & 86M \\
    % ViT-L~\cite{dosovitskiy2021an} \textit{\footnotesize ICLR21} & 76.5 & none & 307M \\
    \midrule
    DeiT-Ti~\cite{Touvron2021TrainingAttention} & 72.2 & none & 5M\\
    CivT-Ti~\cite{Ren2022Co-advise:Distillation} & 74.9 & ensemble & 6M \\
    % Closer Look~\cite{Miles2023ADistillation} & 77.2 & regnet-y-160 & 6M \\
    % TRG~\cite{zhang2023knowledge} \textit{\footnotesize TBDATA23} & 75.5 & ceit-s & 6M \\
    % \emoji{angry} ViTKD~\cite{yang2022vitkd} & 77.8 & regnet-y-160 & 6M \\
    % Manifold~\cite{hao2022learning} & 76.5 & cait-s24 & 6M \\
    DeiT-Ti\alambicdeit ~\cite{Touvron2021TrainingAttention} & 74.5 & regnety-160 & 6M \\
    \myalign{l}{\;\;\;\footnotesize \rotatebox[origin=c]{180}{$\Lsh$} 1000 epochs } & 76.6 & regnety-160 & 6M \\
    DearKD~\cite{chen2022dearkd} & 74.8 & regnety-160 & 6M \\
    \myalign{l}{\;\;\;\footnotesize \rotatebox[origin=c]{180}{$\Lsh$} 1000 epochs } & 77.0 & regnety-160 & 6M \\
    USKD~\cite{yang2023knowledge} & 75.0 & regnety-160 & 6M \\
    Our Method & \textbf{77.2} & regnety-160 & 6M \\
    \midrule
    
    ResNet-50 & 76.5 & none & 25M \\
    FunMatch~\cite{Beyer2022KnowledgeConsistent} & 80.3 & bit-m r152x2 & 25M \\
    $\rotatebox[origin=c]{180}{$\Lsh$}$ 9600 epochs & \textbf{82.8} & bit-m r152x2 & 25M \\
    
    \midrule
    DeiT-S~\cite{Touvron2021TrainingAttention} & 79.8 & none & 22M\\
    CivT-S~\cite{Ren2022Co-advise:Distillation} & 82.0 & ensemble & 22M \\
    DeiT-S\alambicdeit~\cite{Touvron2021TrainingAttention} & 81.2 & regnety-160 & 22M \\
    \myalign{l}{\;\;\;\footnotesize \rotatebox[origin=c]{180}{$\Lsh$} 1000 epochs } & 82.6 & regnety-160 & 22M \\
    DearKD~\cite{chen2022dearkd} & 81.5 & regnety-160 & 22M \\
    \myalign{l}{\;\;\;\footnotesize \rotatebox[origin=c]{180}{$\Lsh$} 1000 epochs } & 82.8 & regnety-160 & 22M \\  
    USKD~\cite{yang2023knowledge} & 80.8 & regnety-160 & 22M \\
    Our Method & \textbf{82.1} & regnety-160 & 22M \\
    \bottomrule
\end{tabular}

==> tables/extra/batch.tex <==
\resizebox{.65\linewidth}{!}{
\begin{tabular}{c|ccc}
    \toprule
    Batch size & 64 & 128 & 256 \\
    \midrule
    Accuracy (\%) & 71.36 & 71.41 & \textbf{71.63} \\
    \bottomrule
\end{tabular}
}

==> tables/extra/cifar.tex <==
% \begin{small}
\setlength\tabcolsep{5pt}
\resizebox{.65\linewidth}{!}{
\begin{tabular}{c|cc}
    \toprule
    \belowrulesepcolor{mygrey}
    \rowcolor{mygrey} Teacher & ResNet32×4 & ResNet50 \\
    \belowrulesepcolor{mygrey}
    \rowcolor{mygrey} Student & ResNet8×4 & MobileNet-V2 \\
    \midrule
    Teacher & 79.42 & 79.34 \\ 
    Student & 72.50 & 64.60 \\ 
    \midrule
    KD & 73.33 & 64.60 \\ 
    CRD & 75.51 & 69.11 \\ 
    ReviewKD & 75.63 & 69.89 \\
    DKD & 76.32 & 70.35  \\
    
    % \midrule

    \aboverulesepcolor{myblue}
    \rowcolor{myblue} Ours & 76.55 & 71.53 \\   
    \aboverulesepcolor{myblue}
    \rowcolor{myblue} Ours + DKD & \textbf{76.95} & \textbf{71.75} \\   
    \aboverulesepcolor{myblue}

    \bottomrule
\end{tabular}
}
% \end{small}

==> tables/imagenet_ablation.tex <==
\begin{tabular}{cccc}
    \toprule
    CP & LR & acc@1 & acc@5 \\
    \midrule
    \xmark & \xmark & - & - \\
    \xmark & \cmark & - & - \\
    \cmark & \xmark & - & - \\
    \cmark & \cmark & - & - \\
    
    % ITRD & \xmark & \xmark & - & - \\
    % ITRD & \xmark & \cmark & - & - \\
    % ITRD & \cmark & \xmark & - & - \\
    % ITRD & \cmark & \cmark & - & - \\
    \midrule
\end{tabular}

==> tables/logsum.tex <==

\begin{tabular}{lc}
    \toprule
    Loss & acc@1 \\
    \midrule
    MSE & 70.03 \\
    \myalign{l}{\;\;\;\footnotesize $\rotatebox[origin=c]{180}{$\Lsh$}$ w/ BN + LogSum}  & \textbf{71.29} \\
    \midrule
\end{tabular}

==> tables/normalisation.tex <==
\begin{tabular}{llc}
    \toprule
    Description & Equation & acc@1 \\
    \midrule
    Batch Norm~\cite{Ioffe2015BatchShift} & $\frac{z_{i,k} - \mu_{k}}{\sqrt{\sigma_k + \epsilon}}$ & \textbf{62.76} \\
    % \myalign{l}{\;\;\;\footnotesize $\rotatebox[origin=c]{180}{$\Lsh$}$ w/ $\mathbf{Z}_t$ only} & & - \\
    L2 & $\frac{z}{\lpnorm{z}_2^2}$ & 57.07 \\
    \stackengine{2pt}{Group Norm~\cite{Wu2018GroupNormalization}}{ \highlight{\footnotesize \textbf{groups = 16}} }{U}{c}{F}{T}{S} & $\frac{z_{i,k} - \mu_{i, s_k} }{\sqrt{\sigma_{i, s_k} + \epsilon}}$ & 59.35 \\
     \myalign{l}{\;\;\;\footnotesize $\rotatebox[origin=c]{180}{$\Lsh$}$ w/ Weight Norm~\cite{Qiao2019Micro-BatchStandardization}} & & 56.41 \\
    \midrule
\end{tabular}

==> tables/projector.tex <==
\begin{tabular}{lc}
    \toprule
    Projector & acc@1 \\
    \midrule
    Linear & \textbf{59.75} \\
    MLP & \\
    \myalign{l}{\;\;\;\footnotesize $\rotatebox[origin=c]{180}{$\Lsh$}$ Hidden Size = 64}  & 58.64 \\
    \myalign{l}{\;\;\;\footnotesize $\rotatebox[origin=c]{180}{$\Lsh$}$  Hidden Size = 512} & 59.49 \\
    \myalign{l}{\;\;\;\footnotesize $\rotatebox[origin=c]{180}{$\Lsh$}$ Hidden Size = 2048} & 59.54 \\
    \midrule
\end{tabular}

==> tables/rebuttal/alpha.tex <==
\renewcommand{\arraystretch}{1.4}
\begin{tabular}{cccccccc}
    \toprule
    % Teacher $\rightarrow$ Student & \multicolumn{6}{c}{$\alpha = $} \\
    % \midrule
    \belowrulesepcolor{mygrey}
    \rowcolor{mygrey} Teacher $\rightarrow$ Student & 1.0 & 1.5 & 2.0 & 2.5 & 3.0 & 4.0 & 5.0\\
    \aboverulesepcolor{mygrey}
    \midrule
    R50 $\rightarrow$ R18 & 61.74 & 62.18 & 62.23 & 62.84 & 63.10 & 63.32 & \textbf{63.40} \\
    ConvNeXt $\rightarrow$ EffNet & 65.52 & 66.69 & 66.61 & 67.10 & 67.72 & \textbf{68.51} & 67.69 \\
    \midrule
\end{tabular}

==> tables/rebuttal/alpha_new.tex <==
% \renewcommand{\arraystretch}{1.4}
\begin{tabular}{cccccc}
    \toprule
    % Teacher $\rightarrow$ Student & \multicolumn{6}{c}{$\alpha = $} \\
    % \midrule
    \belowrulesepcolor{mygrey}
    \rowcolor{mygrey} Teacher $\rightarrow$ Student & 1.0 & 2.0 & 3.0 & 4.0 & 5.0\\
    \aboverulesepcolor{mygrey}
    \midrule
    R50 $\rightarrow$ R18 & 61.74 & 62.23 & 63.10 & 63.32 & \textbf{63.40} \\
    ConvNeXt $\rightarrow$ EffNet & 65.52 & 66.61 & 67.72 & \textbf{68.51} & 67.69 \\
    \midrule
\end{tabular}

==> tables/repulsive_force.tex <==
\begin{tabular}{llcc}
    \toprule
    Description & Repulsive force & acc@1 \\
    \midrule
    \stackengine{2pt}{Mean-square}{ \highlight{\footnotesize \textbf{no projection}} }{U}{c}{F}{T}{S} & $\lpnorm{z_s - z_t}_2^2$ & 71.08 \\
    % \midrule
    Mean-square & $\lpnorm{z_s - z_t}_2^2$ & 71.53 \\
    Batch-normalised & $\lpnorm{ \highlight{BN}(z_s) - \highlight{BN}(z_t) }_2^2$ & 71.34 \\
    Correlation & $\lpnorm{BN(z_s) \cdot BN(z_t) \highlight{- \mathbf{1}} }^2$ & 71.35 \\ 
    Higher-order & $\lpnorm{BN(z_s) \cdot BN(z_t) - \mathbf{1} }^\highlight{4}$ & 71.31 \\ 
    Soft maximum & $\highlight{log \sum} \lpnorm{BN(z_s) \cdot BN(z_t) - \mathbf{1} }^4$ & \textbf{71.63} \\ 
    \midrule
\end{tabular}

==> tables/yolo.tex <==
\begin{tabular}{lcccc}
    \toprule
    Model & mAP (50-95) & mAP 50 & params & FLOPs \\
    \midrule
    YOLOv5m (teacher) & 64.1 & 45.4 & 21.2 & 49.0 \\
    % \midrule
    YOLOv5s & 56.8 & 37.4 & 7.2 & 16.5 \\

    $\rotatebox[origin=c]{180}{$\Lsh$}$ Our Method & \textbf{57.3} & \textbf{37.5} & & \\
    
    \midrule
    & mAP & AP50 & params & \\
    \midrule
    
    Faster R-CNN w/ R50-FPN (teacher) & 40.22 & 61.02 & 41.7 & \\
    % \midrule
    Faster R-CNN w/ MV2-FPN & 29.47 & 48.87 & 23.4 & \\
    $\rotatebox[origin=c]{180}{$\Lsh$}$ KD~\cite{Hinton2015DistillingNetwork} & 30.13 & 50.28 & & \\
    $\rotatebox[origin=c]{180}{$\Lsh$}$ FitNet~\cite{Romero2015FitNets:Nets} & 30.20 & 49.80 & & \\
    $\rotatebox[origin=c]{180}{$\Lsh$}$ FPGI~\cite{Wang2019DistillingImitationb} & 31.16 & 50.68 & & \\
    $\rotatebox[origin=c]{180}{$\Lsh$}$ ReviewKD~\cite{Chen2021DistillingReview} & \textbf{33.71} & \textbf{53.15}  & & \\
    % epoch 299/300
    $\rotatebox[origin=c]{180}{$\Lsh$}$ Our Method & \underline{32.92} & \underline{52.96} & & \\

    \bottomrule
    
\end{tabular}
